Hallucination Augmented Recitations for Language Models

Attribution is a key concept in large language models (LLMs) as it enables control over information sources and enhances the factuality of LLMs. While existing approaches utilize open book question answering to improve attribution, factual datasets may reward language models to recall facts that they already know from their pretraining data, not attribution. In contrast, counterfactual open book QA datasets would further improve attribution because the answer could only be grounded in the given text. We propose Hallucination Augmented Recitations (HAR) for creating counterfactual datasets by utilizing hallucination in LLMs to improve attribution. For open book QA as a case study, we demonstrate that models finetuned with our counterfactual datasets improve text grounding, leading to better open book QA performance, with up to an 8.0% increase in F1 score. Our counterfactual dataset leads to significantly better performance than using humanannotated factual datasets, even with 4x smaller datasets and 4x smaller models. We observe that improvements are consistent across various model sizes and datasets, including multi-hop, biomedical, and adversarial QA datasets.

==> prompts/attribution_filter.tex <==
Given a document, question, and answer pair, the goal is to determine whether the document provides an answer to the question. The answer can be factual or counterfactual, but the goal is to find whether the answer is attributable to the document. Attributable means that the answer must be explicitly stated in the document and should be only inferred from the document.
\\\\
Question: The highest recorded bird strike by an aircraft is a?

Document: A bird strike—sometimes called birdstrike, bird ingestion (for an engine), bird hit, or bird aircraft strike hazard (BASH)—is a collision between an airborne animal (usually a bird or bat) and a moving vehicle, usually an aircraft. The term is also used for bird deaths resulting from collisions with structures such as power lines, towers and wind turbines (see Bird–skyscraper collisions and Towerkill). A significant threat to flight safety, bird strikes have caused a number of accidents with human casualties. There are over 13,000 bird strikes annually in the US alone. However, the number of major accidents involving civil aircraft is quite low and it has been estimated that there is only about 1 accident resulting in human death in one billion (109) flying hours. The majority of bird strikes (65\%) cause little damage to the aircraft; however the collision is usually fatal to the bird(s) involved.

Answer: Bird

Attributable: No
\\\\
Question: What is the last U.S. state, alphabetically?

Document: As of 2018, there are 50 states in the U.S. There are also 14 U.S. territories, but they are not included in the alphabetized list of the 50 U.S. states. The last U.S. state alphabetically is Wisconsin.

Answer: Wisconsin

Attributable: Yes
\\\\
Question: Which colour/color is generally considered between violet and green in the optical spectrum?

Document: The color spectrum is a continuum of wavelengths of light, and what we perceive as color is the way our brain interprets the different wavelengths reflected by objects. The colors of the visible spectrum include red, orange, yellow, green, blue, indigo and violet.

Answer: Indigo

Attributable: No
\\\\
Question: What is the largest ethnic group in Germany (besides Germans)?

Document: Germans (German: Deutsche) are a Germanic ethnic group native to Central Europe, who share a common German ancestry, culture and history. German is the shared mother tongue of a substantial majority of ethnic Germans.  Ethnic Germans are the 2nd largest ancestry group in the United States and have had a major influence on American culture. German Americans are the largest ethnic group in the United States after English Americans.

Answer: Americans

Attributable: No
\\\\
Question: Prior to the coming of William the Conqueror in 1066 where was the capital of England situated?

Document: Prior to the coming of William the Conqueror in 1066, the capital of England was situated in London. William decided to create a new capital at Winchester, which was a great Anglo-Saxon city and royal centre.

Answer: London

Attributable: Yes
\\\\
Question: \{question\}

Document: \{document\}

Answer: \{prediction\}

Attributable:

==> prompts/factuality_filter.tex <==
Given two answers to a question, determine whether they are conflicting or the same. If the two answers lead to the same answer through synonyms, hypernyms, translation, or other related concepts, then respond with "Yes" Otherwise, respond with "No"
\\\\
Question: Which name is associated with the IT developments which grew into Apple?

Answer 1: Jobs

Answer 2: Steve Jobs

Same: Yes
\\\\
Question: What category 3 hurricane devastated the east coast last week, resulting in at least 54 deaths?

Answer 1: Irene

Answer 2: Matthew

Same: No
\\\\
Question: In pre-decimal currency in the UK, how many florins were in a pound?

Answer 1: Ten

Answer 2: 10

Same: Yes
\\\\
Question: Greek jeweller Sotirio Voulgaris founded which luxury goods brand, noted for its capitalized branding including Latin-style V for a U?

Answer 1: Bulgari

Answer 2: Bvlgari

Same: Yes
\\\\
Question: The flags of China, Japan, Argentina, Uruguay, Greenland and Bangladesh share what common feature?

Answer 1: Sun

Answer 2: Circle

Same: No
\\\\
Question: In 1956, a major uprising in Hungary was put down by forces from where?

Answer 1: USSR

Answer 2: Soviet

Same: Yes
\\\\
Question: How many dots make up the BlackBerry symbol logo?

Answer 1: Seven

Answer 2: 22

Same: No
\\\\
Question: Ted Dexter was a Cambridge blue at two sports, cricket was one what was the other

Answer 1: Golf

Answer 2: Rugby

Same: No
\\\\
Question: \{question\}

Answer 1: \{gold\}

Answer 2: \{prediction\}

Same:

==> prompts/generation.tex <==
\begin{quote}
Question: In which Scandinavian city are the headquarters of the Volvo manufacturing company?

Instruction 1: The answer to the above question can be found in the following document.

Document: The Volvo Group is one of the world’s leading manufacturers of trucks, buses, construction equipment and marine and industrial engines. The Group also provides complete solutions for financing and service. The Volvo Group, with its headquarters in Gothenburg, employs about 100,000 people, has production facilities in 18 countries and sells its products in more than 190 markets.

Instruction 2: Answer the given question based on the above document.

Answer: Gothenburg
\\\\
Question: Who was President Reagan's Secretary for Defense from 1987 to 1989?

Instruction 1: The answer to the above question can be found in the following document.

Document: The Secretary of Defense manages all the armed forces of the United States. The Army, Navy, Air Force, Marines, National Guard, and Reserve Forces are part of this Department. Frank C. Carlucci was appointed to the position of Secretary of Defense by President Ronald Reagan in 1987 and served until 1989.

Instruction 2: Answer the given question based on the above document.

Answer: Frank Carlucci
\\\\
Question: Awarded to applicants annually since 1902, the Rhodes Scholarships are for study at what institution?

Instruction 1: The answer to the above question can be found in the following document.

Document: The Rhodes Scholarship, named after Cecil John Rhodes, is an international postgraduate award for study at Oxford University. Rhodes Scholarships have been awarded to applicants annually since 1902 on the basis of academic achievement and strength of character. Thirteen Hale School students have won the award, four of whom have had the honour of having Junior School Houses (Turnbull, Davy, Rosier and Walker) named after them and one Senior School House (Riley). The editor of the Cygnet in March 1908, when writing about the School’s disappointment that H.N. Walker had not won the scholarship that year, pointed out that the Rhodes selectors had to take into consideration not only scholarship but also proficiency in games, character, capacity for leadership, and personality generally.

Instruction 2: Answer the given question based on the above document.

Answer: University of Oxford
\\\\
Question: The Man Booker prize is awarded for what?

Instruction 1: The answer to the above question can be found in the following document.

Document: The Man Booker Prize for Fiction is a literary prize awarded each year for the best novel originally written in English and published in the UK in the The Man Booker Prize for Fiction is a literary prize awarded each year for the best novel originally written in English and published in the UK in the year of the prize, regardless of the nationality of their author. The novel must be an original work in English (not a translation) and must not be self-published. Prior to 2014, eligibility for the award was restricted to citizens of the Commonwealth of Nations, Ireland, or Zimbabwe. The winner of the Man Booker Prize is generally assured of international renown and success; therefore, the prize is of great significance for the book trade. In contrast to literary prizes in the United States, the Booker Prize is greeted with great anticipation and fanfare. It is also a mark of distinction for authors to be selected for inclusion in the shortlist or even to be nominated for the longlist.

Instruction 2: Answer the given question based on the above document.

Answer: Literature
\\\\
Question: What Revolutionary War hero, who regretted that he had but one life to give his country, was hung by the British on Sept 22, 1776?

Instruction 1: The answer to the above question can be found in the following document.

Document: "I only regret that I have but one life to lose for my country." Have you heard this famous declaration before? American patriot Nathan Hale said it on September 22, 1776, his last words before he was hanged for spying on British troops. How did this come to pass? Hale, born in Coventry, Connecticut, on June 6, 1755, and a teacher by trade, joined his five brothers in the fight for independence against the British.

Instruction 2: Answer the given question based on the above document.

Answer: Nathan Hale
\\\\
Question: \{question\}

Instruction 1: The answer to the above question can be found in the following document.
\end{quote}

